Black-Box Adversarial Attacks on LLM-Based Code Completion

Modern code completion engines, powered by large language models (LLMs), assist millions of developers with their strong capabilities to generate functionally correct code. Due to this popularity, it is crucial to investigate the security implications of relying on LLM-based code completion. In this work, we demonstrate that state-of-the-art black-box LLM-based code completion engines can be stealthily biased by adversaries to significantly increase their rate of insecure code generation. We present the first attack, named INSEC, that achieves this goal. INSEC works by injecting an attack string as a short comment in the completion input. The attack string is crafted through a query-based optimization procedure starting from a set of carefully designed initialization schemes. We demonstrate INSEC's broad applicability and effectiveness by evaluating it on various state-of-the-art open-source models and black-box commercial services (e.g., OpenAI API and GitHub Copilot). On a diverse set of security-critical test cases, covering 16 CWEs across 5 programming languages, INSEC increases the rate of generated insecure code by more than 50%, while maintaining the functional correctness of generated code. We consider INSEC practical -- it requires low resources and costs less than 10 US dollars to develop on commodity hardware. Moreover, we showcase the attack's real-world deployability, by developing an IDE plug-in that stealthily injects INSEC into the GitHub Copilot extension.

==> figures/sc2_results/figure.tex <==
\begin{figure*}
  \resizebox*{\columnwidth}{!}{
  \begin{tikzpicture}
    \begin{groupplot}[
      height=3.6cm, width=14cm,
      /pgf/bar width=0.35cm,
      axis x line*=bottom, axis y line*=left, enlarge x limits=true,
      xtick={0, 1},
      xticklabel style={yshift=-0.8mm, font=\footnotesize, align=center},
      ybar=5pt,
      ymin=0, ymax=103, ytick={0, 25, 50, 75, 100}, yticklabels={0, 25, 50, 75, 100},
      ymajorgrids, major grid style={draw=black!20}, tick align=inside,
      yticklabel style={font=\scriptsize}, tickwidth=0pt,
      y axis line style={opacity=0},
      nodes near coords={\pgfmathprintnumber[precision=0]{\pgfplotspointmeta}},
      every node near coord/.append style={font=\scriptsize},
      group style={group size=1 by 2, horizontal sep=30pt, vertical sep=30pt},
      legend style={
        at={(1.2,-0.08)},  % Position of the legend
        anchor=south,  % Anchor point of the legend
        legend columns=1,  % Number of columns in the legend (-1 means that all entries are in one row)
        draw=none,
        row sep=0.1cm,
        column sep=0.1cm,
      },
      legend image code/.code={%
        \draw[#1, draw=mydrawgray] (0cm,-0.125cm) rectangle (0.5cm,0.125cm);
      },
      legend cell align={left},
    ]

      \nextgroupplot[
        xmin=-0.1, xmax=2.2,
        xtick={0, 1, 2},
        xticklabels={\scodertwoThreeB{}, \scodertwoSevenB{}, \scodertwoFifteenB{}},
      ]

        \addplot [draw=mydrawgray, line width=0.7pt, fill=baselineVulColor] table [x=model, y=baselineVR, col sep=comma] {figures/sc2_results/data.csv};
        \addlegendentry{\small $\vulratio(\engine)$}

        \addplot [draw=mydrawgray, line width=0.7pt, fill=optVulColor] table [x=model, y=optVR, col sep=comma] {figures/sc2_results/data.csv};
        \addlegendentry{\small $\vulratio(\engineadv)$}

        \addplot [draw=mydrawgray, line width=0.7pt, fill=pass1Color] table [x=model, y=pass@1, col sep=comma] {figures/sc2_results/data.csv};
        \addlegendentry{\small $\funcratioone(\engineadv, \engine)$}

        \addplot [draw=mydrawgray, line width=0.7pt, fill=pass10Color] table [x=model, y=pass@10, col sep=comma] {figures/main_results/data.csv};
        \addlegendentry{\small $\funcratioten(\engineadv, \engine)$}
  
    \end{groupplot}
  \end{tikzpicture}
  }
  \caption{Experimental results across varyingly sized member models of the \scodertwo{} family. While \tool{} achieves strong results across all model sizes, as the model size increases, both the vulnerability rate and the functional correctness of the attacked engines increases. This result is concerning, as it shows that more capable code completion engines are strongly susceptible to \tool{}-style black-box adversarial attacks.}
  \label{fig:sc2_results}

\end{figure*}
